Upper Confidence Bounds for Combining Stochastic Bandits

We provide a simple method to combine stochastic bandit algorithms. Our approach is based on a "meta-UCB" procedure that treats each of $N$ individual bandit algorithms as arms in a higher-level $N$-armed bandit problem that we solve with a variant of the classic UCB algorithm. Our final regret depends only on the regret of the base algorithm with the best regret in hindsight. This approach provides an easy and intuitive alternative strategy to the CORRAL algorithm for adversarial bandits, without requiring the stability conditions imposed by CORRAL on the base algorithms. Our results match lower bounds in several settings, and we provide empirical validation of our algorithm on misspecified linear bandit and model selection problems.

==> doublinggap.tex <==
\subsection{Doubling Trick for Gap-Dependent Logarithmic Regret}

Next, we show that this same duplication and doubling method works well to preserve our gap-dependent bound in Section \ref{sec:gap}. Of particular interest is the case of \emph{logarithmic} regret, in which each algorithm $\A_i$ attempts to guarantee expected regret after $T$ iterations of $O\left(\frac{\log(T)}{\Delta_i}\right)$ for some unknown parameter $\Delta_i$. For example, consider the following scenario studied by \cite{arora2020corralling}. We have a multi-armed bandit problem in which each $\A_i$ is restricted to different subsets of the arms. Suppose $\A_J$ is the sole algorithm that considers the true optimal arm, and let $\Delta$ be the gap between the expected reward of the optimal and the second-best arm. Then if $\A_J$ is a standard UCB algorithm, we could describe it as having as a putative anytime regret bound after $t$ iterations of $C_Jt^{\alpha_i}$ with $C_J=O\left(\frac{\log(T)}{\Delta_J}\right)$ and $\alpha_i=0$, and set $R_J=C_JT^{\alpha_J}$. Further, suppose all the other algorithms guarantee $C_i\sqrt{t}$ regret for their some $C_i$ and let $\Delta_i$ be the gap between the best arm available to $\A_i$ and the true best arm. Then Theorem \ref{thm:gap} would imply a regret of:
\begin{align*}
    \tilde O\left[\frac{1}{\Delta_J} + \sum_{i\ne J}\frac{C_i^2}{\Delta_i}\right]
\end{align*}
Suppressing the log factors, this matches the bound provided by \cite{arora2020corralling}. However, there are two issues here: first, the typical logarithmic regret bound is an in-expectation bound rather than a high-probability bound, and second, we do not know the value of $\Delta_J$ required to tune $C_J$. We show that, at the expense of log factors, the doubling and duplication trick can overcome these obstacles. This method is performing an intuitively similar operation to the duplication and median procedure used by \cite{arora2020corralling}. Specifically, we have the following:
\begin{restatable}{Theorem}{thmdoublinggap}\label{thm:doublinggap}

Suppose that for some $J$, there is some unknown $\bar C_J$ and $\bar \alpha_J$ such that $\A_J$ ensures $\E[\sum_{\tau=1}^t r_\star - r^J_\tau]\le \bar C_Jt^{\bar\alpha_J}$ for all $t \leq T$. Let $\delta \in (0,1)$ be some user-specified failure probability. For $M=\lceil \log_2(1/\delta)\rceil$ and $K=\lceil \log_2(T)\rceil$ and $L=\lceil\frac{\log_2(T)}{2}\rceil$, we duplicate each $\A_i$ $MKL$ times, specifying each duplicate $\A_{i,x,y,z}$ by a multi-index 
\end{restatable}
